Linear Bandits with Non-i.i.d. Noise

We study the linear stochastic bandit problem, relaxing the standard i.i.d. assumption on the observation noise. As an alternative to this restrictive assumption, we allow the noise terms across rounds to be sub-Gaussian but interdependent, with dependencies that decay over time. To address this setting, we develop new confidence sequences using a recently introduced reduction scheme to sequential probability assignment, and use these to derive a bandit algorithm based on the principle of optimism in the face of uncertainty. We provide regret bounds for the resulting algorithm, expressed in terms of the decay rate of the strength of dependence between observations. Among other results, we show that our bounds recover the standard rates up to a factor of the mixing time for geometrically mixing observation noise.

==> proof.tex <==

\subsection{Proof of Theorem \ref{thm:conf_seq_iid}}

\begin{proof}
For each $t \geq 1$, we choose the comparator to be $\wh\theta_t$. From \Cref{thm:standard_otcs}, the regret bound in Proposition \ref{pro:uniform_ewa_regret} and the fact that $\|\theta^{\star}\|_2 \leq B$, we know that for any $\lambda \geq 0$,
\begin{equation*}
\mathbb{P}\left(\forall t \geq 1, \sum_{s=1}^{t}\ell_s(\theta^{\star}) + \tfrac{\lambda}{2}\|\theta^{\star}\|_2^2 - \sum_{s=1}^{t}\ell_s(\wh\theta_t) \leq \tfrac{p}{2}\log\tfrac{(B+1)^2e\max(p, t)}{p} + \tfrac{\lambda}{2}\|\theta^{\star}\|_2^2 + \log\tfrac{1}{\delta}\right) \geq 1 - \delta\,.
\end{equation*}

By taking a second-order Taylor expansion of $\sum_{s=1}^{t}\ell_s(\theta) + \frac{\lambda}{2}\|\theta\|_2^2$ around $\wh\theta_t$, we obtain
\begin{equation*}
\sum_{s=1}^{t}\ell_s(\theta^{\star}) + \tfrac{\lambda}{2}\|\theta^{\star}\|_2^2 - \sum_{s=1}^{t}\ell_s(\wh\theta_t) = \tfrac{\lambda}{2}\|\wh\theta_t\|_2^2 + \iprod{\theta^{\star} - \wh\theta_t}{\lambda \wh\theta_t + \nabla\sum_{s=1}^{t}\ell_s(\wh\theta_t)} + \tfrac{1}{2}\|\theta^{\star} - \wh\theta_t\|_{V_t}^2\,.
\end{equation*}

Using the first-order optimality condition, we have that $\siprod{\theta^{\star} - \wh\theta_t}{\nabla\sum_{s=1}^{t}\ell_s(\wh\theta_t)} \geq 0$. Therefore, after a bit of algebra, the previous two equations tell us that
\begin{equation*}
\mathbb{P}\left(\forall t \geq 1, \|\theta^{\star} - \wh\theta_t\|_{V_t}^2 \leq p\log\tfrac{(B+1)^2e\max(p,t)}{p} + 2\lambda B^2 + 2\log\tfrac{1}{\delta}\right) \geq 1 - \delta\,.
\end{equation*}

Thus, the sets defined in the statement of the theorem form a confidence sequence for $\theta^{\star}$.
\end{proof}



\begin{proof}
    Let define for $s \in[t], \lambda_s := \siprod{X_s}{\theta_s-\theta^*}$. Denote $g_s(\theta^*):=\ell_s(\theta^*)-\ell_s(\theta_s)$ and remark that $g_s(\theta^*)=-\frac{\lambda_s^2}{2}+\lambda_s\epsilon_s.$
    \begin{align*}
        \EEc{W_t}{\F_{t-1}}&= W_{t-1}\EEc{e^{-\frac{\lambda_t^2}{2}+\lambda_t\epsilon_t}}{\F_{t-1}}\\ 
        &\leq W_{t-1}e^{\frac{(\sigma^2-1)\lambda_t^2}{2}} \qquad \text{($\sigma$-subgaussianity of } \epsilon_t)\\
        &\leq W_{t-1} \qquad \text{(for } \sigma\leq 1) 
    \end{align*}
\end{proof}
\subsection{Lemma \ref{lemma:mixing_concentration_bound}}
\begin{lemma}
\label{lemma:mixing_concentration_bound}
    For any $t$ and $d \leq t$ with probability $1-\delta$:
    \[ M_t(\theta^*)-Ct\phi_d \leq d \log\frac{d}{\delta},\]
    where $C:=2\sup_{x,\theta} \siprod{x}{\theta}$
\end{lemma}
\begin{proof}
We use 
\begin{align*}
\mathbb{P}(\forall t \geq d, M_t \leq d\log(1/\delta)) &\geq \mathbb{P}\left(\cap_{i \in [d]}[\forall k \geq 1]\right)
\end{align*}

\bapt{Hamish is gonna write a new version of this proof.}
\label{proof::lemma_mixing_concentration_bound}
We are gonna split the proof in two cases.

\textbf{Case $t=Kd$}


   Let $K =\frac{t}{d}$. Then we can rewrite $M_t$ as:
   \[M_t = \sum_{i=1}^d M_K^i\] where $M_K^i = \sum_{k=1}^K \ell_{k}^i(\theta^*)-\ell_{k}^i(\theta_{k}^i)$ and denote the event $A_t(\delta) := [M_t(\theta^*) - Ct\phi_d \leq d \log \frac{1}{\delta}].$ Then 
    \begin{align*}
        \mathbb{P}(A_t) &\geq \mathbb{P}\left(\bigcap_{i \in [d]} \left[M_K^i-CK\phi_d \leq \log \frac{1}{\delta} \right]\right)\\
        &\geq 1 -\mathbb{P}\left(\bigcup_{i \in [d]} \left[M_K^i-CK\phi_d > \log \frac{1}{\delta}  \right]\right) \\
        &\geq 1-d\delta \qquad (\text{this last inequality comes from Lemma \ref{lemma::SMG_mixing})}
    \end{align*}
    Setting $\delta'=\frac {\delta}{d}$ and applying the above  with $A_t(\delta')$ yields the final result.
    
  \textbf{Case $t=(K-1)d + r:$}

\end{proof}
\subsection{Proof of Lemma \ref{lemma::SMG_mixing}}


\label{proof:SMG_mixing}
 

Let $t > 0$, we are gonna decompose the proof in 2 cases.  Either $t=Kd$ or $t = (K-1)d + r$, with $d>r>0$.

\textbf{Case $t=Kd$}:
In this case we can directly rewrite
$$M_t = \sum_{i=1}^dM_K^i$$
where $M_K^i= \sum_{k=1}^K g_k^i$ where $g_k^i$ is a shorthand for $g_{i+(k-1)d}$. Now let define for $k\in [K-1]$ the filtration $\F_k^i:= \sigma(x_i,\epsilon_i,X_{i+d},\epsilon_{i+d},\dots,,X_{i+(k-1)d},\epsilon_{i+(k-1)d},X_{i+kd})$ and prove that for any $k \in [K]$,
$$\EE{e^{M_k^i-kC\phi_d}|\F_{k-1}^i}\leq e^{M_{k-1}^i-(k-1)C\phi_d}.$$
The proof of the above statement is established below for $k=K.$
\begin{align*}
    \EE{e^{M_K^i-KC\phi_d}|\F_{K-1}^i}&=e^{M_{K-1}^i-(K-1)C\phi_d}\EEc{e^{g_K^i-C\phi_d}}{\F_{K-1}^i}\\
    &= e^{M_{K-1}^i-(K-1)C\phi_d}\EEc{e^{-\frac{(\lambda_K^i)^2} {2}+\lambda_K^i\epsilon_K^i-C\phi_d}}{\F_{K-1}^i}\\
    &= e^{M_{K-1}^i-(K-1)C\phi_d}e^{-\frac{(\lambda_K^i)^2}{2}-C\phi_d}\EEc{e^{\lambda_K^i\epsilon_K^i}}{\F_{K-1}^i} \qquad \text{(because $\lambda_K^i$ is $\F_{K-1}^i$-measurable*)}\\
    &=e^{M_{K-1}^i-(K-1)C\phi_d}e^{-\frac{(\lambda_K^i)^2}{2}-C\phi_d}\underbrace{\EEc{e^{\lambda_K^i\left(\epsilon_K^i-\EEc{\epsilon_K^i}{\F_{K-1}^i}\right)}}{\F_{K-1}^i}}_{(1)}\underbrace{e^{\lambda_K^i\EEc{\epsilon_K^i}{\F_{K-1}^i}}}_{(2)}
\end{align*}

(*) This bit is fundamental in the design of our algorithm so we want to shed the light on why it's true. By definition $\lambda_K^i:= \siprod{X_K^i}{\theta_K^i-\theta^*}$, so it is enough is to assume that both $x_K^i$ and $\theta_K^i$ are $\F_{K-1}^i$-measurable. The former is clearly stated in the assumption of Lemma \ref{lemma::SMG_mixing}, the latter is justified because of the delay incurred by online learner in the abstract game . 
 
To bound $(2)$ we use assumption \ref{eq::mixing}, this implies that $(2) \leq e^{|\lambda_K^i|\phi_d}$. Recall that $\lambda_t:=\siprod{X_t}{\theta_t-\theta^*}$ and we can reasonably assume that $|\lambda_t| \leq C$ for all $t$ (this amounts to saying that $\X$ and $\Theta$ are bounded). To bound $(1)$ we apply Assumption \ref{ass:mixing-subgaussianity}.
Combining everything it follows that:
\begin{align*}
     \EE{e^{M_K^i-KC\phi_d}|\F_{K-1}^i} \leq e^{M_{K-1}^i-(K-1)C\phi_d}.
\end{align*}

\textbf{Case $t=(K-1)d + r$ with $0<r<d$:} 

In this case we can no longer rewrite $M_t$ as a sum over each block $M_t := \sum_{i=1}^d M_K^i$
    where $M_K^i := \sum_{k=1}^K g_{i+(k-1)d}$, because $g_{i+(K-1)d}$ is  not defined for $i>r$. Therefore we are gonna decompose it into two sums, those of length $K$ and those of length $K-1$. Formally:
    $$M_t := \sum_{i=1}^r M_K^i + \sum_{i=r+1}^d M_{K-1}^i$$
    and apply the result of the first case to each block.

\subsection{Randomised Online Learning Algorithms/Sequential Probability Assignment in the standard setting}
\label{sec:ewa}

We can build a confidence sequence using the outputs $\theta_1, \theta_2, \dots$ of an algorithm for online squared error regression using the regret plus log of martingale decomposition
\begin{equation*}
\sum_{s=1}^t\ell_t(\theta^*)-\ell_s(\wh \theta_t) = \underbrace{\sum_{s=1}^t \ell_s(\theta_s)-\ell_s(\wh \theta_t) }_{\text{regret term}}  + \underbrace{\sum_{s=1}^t \ell_s(\theta^*)-\ell_s(\theta_s)}_{\text{log martingale term}}\,.
\end{equation*}
\begin{lemma} If we assume $(\epsilon_t)$ conditionally zero-mean and 1-sub-Gaussian, then
    \label{lemma:Concentration_SMG_classic}
    $M_t:=e^{\sum_{s=1}^t \ell_s(\theta^*)-\ell_s(\theta_s)}$ is a supermartingale w.r.t $\F_t$.
\end{lemma}
\begin{proof}
    We denote for $t>0, \lambda_t(\theta) = \langle \theta_t -\theta^\star, X_t\rangle$ and remark that $\ell_t(\theta^*)-\ell_t(\theta_t) = -\frac{\lambda_t(\theta^*)^2}{2}+\lambda_t(\theta^*)\epsilon_t$ We have 
    \begin{align*}
        \EEc{M_t}{\F_{t-1}}&= M_{t-1}\EEc{e^{-\frac{\lambda_t(\theta^*)^2}{2}+\lambda_t(\theta^*)\epsilon_t}}{\F_{t-1}}\\
        &=M_{t-1}e^{-\frac{\lambda_t(\theta^*)^2}{2}}\EEc{e^{\lambda_t(\theta^*)\epsilon_t}}{\F_{t-1}} \\
        &\leq M_{t-1}.
    \end{align*}
The second equality holds because $\lambda_t(\theta^*)$ is $\F_{t-1}$-measurable. The inequality is due to the 1-sub-Gaussianity of $\epsilon_t$ which implies that $\EEc{e^{\lambda_t(\theta^*)\epsilon_t}}{\F_{t-1}}\leq e^{\frac{\lambda_t(\theta^*)^2}{2}}.$
\end{proof}

The best known bounds on this regret term are of order $\mathcal{O}(\max_{s \in [t]}Y_s^2 p\log(t))$. The maximum squared label can be bounded by a constant times $\log(t)$, so we get $\mathcal{O}(p\log(t)^2)$. However, we would like the RHS to be of order $\mathcal{O}(p\log(t))$. We can remove the dependence on the max label by switching to randomised online learning algorithms, which return a sequence of distributions $Q_1, Q_2, \dots, $ on the set of parameter vectors. We define $\mathcal{L}_s(Q) = -\log(\int\exp(-\ell_s(\theta))\mathrm{d}Q(\theta))$, which is sometimes called the log loss. We can then write
\begin{equation}
\sum_{s=1}^t\ell_s(\theta^*)-\ell_s(\wh \theta_t) = \underbrace{\sum_{s=1}^t \mathcal{L}_s(Q_s)-\ell_s(\wh \theta_t) }_{\text{regret term}}  + \underbrace{\sum_{s=1}^t \ell_s(\theta^*)-\mathcal{L}_s(Q_s)}_{\text{log martingale term}}\label{eqn:randomised_reg_plus_mart}
\end{equation}

As long as the distributions $(Q_s)_{s \in \mathbb{N}}$ are predictable w.r.t.\ $(\mathcal{F}_s)_{s \in \mathbb{N}}$, then the log martingale term is still the log of a non-negative supermartingale. If we let $M_t = \exp(\sum_{s=1}^{t}\ell_s(\theta^*) - \mathcal{L}_s(Q_s))$, then by using the fact that each $Q_s$ is $\mathcal{F}_{s-1}$-measurable,
\begin{align*}
\mathbb{E}[M_t|\mathcal{F}_{t-1}] &= M_{t-1}\mathbb{E}[\exp(\ell_t(\theta^*) - \mathcal{L}_t(Q_t))|\mathcal{F}_{t-1}]\\
&= M_{t-1}\mathbb{E}\left[\int\exp(\ell_t(\theta^*) - \ell_t(\theta))\mathrm{d}Q_t(\theta)\Big|\mathcal{F}_{t-1}\right]\\
&= M_{t-1}\int\mathbb{E}[\exp(\ell_t(\theta^*) - \ell_t(\theta))|\mathcal{F}_{t-1}]\mathrm{d}Q_t(\theta)\\
&\leq M_{t-1}\,,
\end{align*}

where the last inequality follows from the proof of Lemma \ref{lemma:Concentration_SMG_classic} (which shows that $\mathbb{E}[\exp(\ell_t(\theta^*) - \ell_t(\theta))|\mathcal{F}_{t-1}] \leq 1$). The regret term is now the regret of $(Q_s)_{s \in [t]}$ in a problem called \emph{sequential probability assignment}. There are algorithms for sequential probability assignment that have regret of order $\mathcal{O}(p\log(t/p))$, which gives us a RHS with the right dependence on $p$ and $t$. In this setting, if we use the Exponentially Weighted Average (EWA) forecaster to generate $Q_1, Q_2, \dots$, then we can write down a closed-form expression for this regret term. The EWA forecaster (with learning rate 1) is defined by
\begin{equation*}
\frac{\mathrm{d}Q_t}{\mathrm{d}Q_1}(\theta) = \frac{\exp(-\sum_{s=1}^{t-1}\ell_s(\theta))}{\int \exp(-\sum_{s=1}^{t-1}\ell_s(\theta))\mathrm{d}Q_1(\theta)}\,.
\end{equation*}

Since $\ell_t$ is the negative log likelihood (if the noise was actually Gaussian), this is equivalent to Bayesian linear regression. Using the definition of $Q_t$, we can write the total log loss as
\begin{align*}
\sum_{t=1}^{n}\mathcal{L}_t(Q_t) &= \sum_{t=1}^{n}-\log\int\exp(-\ell_t(\theta))\mathrm{d}Q_t(\theta)\\
&= \sum_{t=1}^{n}-\log\left(\frac{\int \exp(-\sum_{s=1}^{t}\ell_s(\theta))\mathrm{d}Q_1(\theta)}{\int \exp(-\sum_{s=1}^{t-1}\ell_s(\theta))\mathrm{d}Q_1(\theta)}\right)\\
&= -\log\int \exp\left(-\sum_{t=1}^{n}\ell_t(\theta)\right)\mathrm{d}Q_1(\theta)\,.
\end{align*}

By subtracting $\sum_{s=1}^{t}\ell_s(\wh\theta_t)$ from both sides, we see that the regret term is
\begin{equation}
\sum_{s=1}^{t}\mathcal{L}_s(Q_s) - \sum_{s=1}^{t}\ell(\wh\theta_t) = -\log\int \exp\left(-\sum_{s=1}^{t}\ell_t(\theta) + \sum_{s=1}^{t}\ell_t(\wh\theta_t)\right)\mathrm{d}Q_1(\theta)\,.\label{eqn:ewa_regret}
\end{equation}

If $Q_1$ is Gaussian, this integral can be evaluated using the Gaussian integral formula (see next Section).


\subsection{Regularised Confidence Sets}
\label{sec:regularised_sets}

We know how to design confidence sets of the form
\begin{equation*}
\Theta_t = \left\{\theta: \sum_{s=1}^{t}\ell_s(\theta) - \sum_{s=1}^{t}\ell_s(\wh \theta_t) \leq \beta_t(\delta)\right\}\,.
\end{equation*}

For the bandit analysis, it is convenient to re-write this set such that the constraint is
\begin{equation*}
\|\theta - \wh \theta_n\|_{V}^2 \leq \wt\beta_n(\delta)\,,
\end{equation*}

where $V$ is some positive (semi-)definite matrix. Since $\sum_{t=1}^{n}\ell_t(\theta)$ is a quadratic function of $\theta$, it's second-order Taylor expansion has remainder 0. Therefore,
\begin{equation*}
\sum_{s=1}^{t}\ell_s(\theta) - \sum_{s=1}^{t}\ell_s(\wh\theta_t) = \iprod{\theta - \wh\theta_t}{\nabla\sum_{s=1}^{t}\ell_s(\wh\theta_t)} + \frac{1}{2}\|\theta - \wh\theta_t\|_{\nabla^2\sum_{s=1}^{t}\ell_s(\wh\theta_t)}^2\,.
\end{equation*}

Since, $\wh\theta_n$ is a minimiser of $\sum_{s=1}^{t}\ell_s(\theta)$, $\nabla\sum_{s=1}^{t}\ell_s(\wh\theta_t)$. For any $\theta$, $\nabla^2\sum_{s=1}^{t}\ell_s(\theta) = \sum_{s=1}^{t}X_sX_s^{\top}$. Therefore, letting $\Lambda_t = \sum_{s=1}^{t}X_sX_s^{\top}$, the original set defined in terms of losses is the same as
\begin{equation*}
\Theta_t = \left\{\theta: \|\theta - \wh \theta_t\|_{\Lambda_t}^2 \leq 2\beta_t(\delta)\right\}\,.
\end{equation*}

However, for the elliptical potential stuff in the next section, we need a confidence set like this where the matrix $\Lambda_n$ is replaced by $V_t= \Lambda_t + \lambda I$, which is always strictly positive definite. We can replace $\Lambda_n$ with $V_t$ by using regularised losses. We define $\wh\theta_{t,\lambda} := \argmin_{\theta \in \real^d}\{\sum_{s=1}^{t}\ell_s(\theta) + \frac{\lambda}{2}\|\theta\|_2^2\}$ to be the minimiser of the regularised loss. Since the regularised loss is still quadratic in $\theta$, and $\nabla^2[\sum_{s=1}^{t}\ell_s(\theta) + \frac{\lambda}{2}\|\theta\|_2^2] = V_t$, another Taylor expansion tells us that
\begin{equation}
\sum_{s=1}^{t}\ell_s(\theta) + \frac{\lambda}{2}\|\theta\|_2^2 - \sum_{s=1}^{t}\ell_t(\wh\theta_{t,\lambda}) + \frac{\lambda}{2}\|\wh\theta_{t,\lambda}\|_2^2 = \frac{1}{2}\|\theta - \wh\theta_{t,\lambda}\|_{V_t}^2\,.
\label{eqn:reg_loss_taylor}
\end{equation}

We will also use the following Gaussian integral formula:
\begin{equation*}
\int_{\real^p}\exp\left(-\tfrac{1}{2}\|\theta - \mu\|_{\Sigma^{-1}}^2\right)\mathrm{d}\theta = \sqrt{(2\pi)^d\det(\Sigma)}\,.
\end{equation*}

Using these two equations (as well as Equation \eqref{eqn:ewa_regret}), we can evaluate the regret of EWA (with the prior $Q_1 = \mathcal{N}(0, \frac{1}{\lambda}I)$) against $\wh\theta_{n,\lambda}$ as
\begin{align*}
\sum_{s=1}^t \mathcal{L}_s(Q_s)-\ell_t(\wh \theta_t) &= -\log\int \exp\left(-\sum_{s=1}^{t}\ell_t(\theta) + \sum_{s=1}^{t}\ell_t(\wh\theta_t)\right)\mathrm{d}Q_1(\theta)\\
&= -\log\left(\frac{\int_{\real^p}\exp(-\sum_{s=1}^{t}\ell_s(\theta) - \frac{\lambda}{2}\|\theta\|_2^2 + \sum_{s=1}^{t}\ell_s(\wh\theta_t))\mathrm{d}\theta}{\int_{\real^p}\exp(-\frac{\lambda}{2}\|\theta\|_2^2)\mathrm{d}\theta}\right)\\
&= -\log\left(\frac{\int_{\real^p}\exp(-\frac{1}{2}\|\theta - \wh\theta_{t,\lambda}\|_{V_t}^2)\mathrm{d}\theta}{\int_{\real^p}\exp(-\frac{\lambda}{2}\|\theta\|_2^2)\mathrm{d}\theta}\right) + \frac{\lambda}{2}\|\wh\theta_{t,\lambda}\|_2^2\\
&= \frac{1}{2}\log\det(\tfrac{1}{\lambda}\Lambda_t + I) + \frac{\lambda}{2}\|\wh\theta_{t,\lambda}\|_2^2\,.
\end{align*}

Combining this with Equation \eqref{eqn:randomised_reg_plus_mart}, and the $\log(1/\delta)$ bound on the martingale term, we obtain
\begin{equation*}
\mathbb{P}\left(\forall t \geq 1, ~\sum_{s=1}\ell_s(\theta^*) - \sum_{s=1}^{t}\ell_t(\wh\theta_{t,\lambda}) \leq \frac{1}{2}\log\det(\tfrac{1}{\lambda}\Lambda_t + I) + \frac{\lambda}{2}\|\wh\theta_{t,\lambda}\|_2^2 + \log\frac{1}{\delta}\right) \geq 1 - \delta
\end{equation*}

If we add $\frac{\lambda}{2}\|\theta^*\|_2^2 - \frac{\lambda}{2}\|\wh\theta_{t,\lambda}\|_2^2$ to both sides, assume that $\|\theta^*\|_2 \leq B$ and use Equation \eqref{eqn:reg_loss_taylor}, then this becomes
\begin{equation*}
\mathbb{P}\left(\forall t \geq 1, ~\|\theta^* - \wh\theta_{t,\lambda}\|_{V_t}^2 \leq \log\det(\tfrac{1}{\lambda}\Lambda_t + I) + \lambda B^2 + 2\log\frac{1}{\delta}\right) \geq 1 - \delta
\end{equation*}

Therefore, we can use
\begin{equation*}
\Theta_t = \left\{\theta: \|\theta - \wh\theta_{t,\lambda}\|_{V_t}^2 \leq \log\det(\tfrac{1}{\lambda}\Lambda_t + I) + \lambda B^2 + 2\log\frac{1}{\delta}\right\}\,.
\end{equation*}

If we choose $\lambda = 1/B^2$, then the squared radius of the confidence set is
\begin{equation*}
\beta_n = \log\det(B^2\Lambda_t + I) + 1 + 2\log\frac{1}{\delta} \geq 1\,.
\end{equation*}

If we also assume that $\max_{s}\|X_s\|_2 \leq L$, then the Determinant-Trace Inequality from \citet{abbasi2011improved} tells us that $\log\det(\tfrac{1}{\lambda}\Lambda_t + I) \leq p\log(1 + \frac{tL^2}{\lambda p})$, which means we get $\beta_t \leq p\log(1 + \frac{tB^2L^2}{p})  + 1 + 2\log\frac{1}{\delta}$, which is of order $\mathcal{O}(p\log(n/p))$. For $t=0$, we can define $\Theta_0$ the be the $\ell_2$ ball of radius $B$, or equivalently
\begin{equation*}
\Theta_0 = \left\{\theta: \|\theta - \wh\theta_{0,1/B^2}\|_{V_0}^2 \leq \beta_0\right\}\,,
\end{equation*}

where $\beta_0 = 1$, $V_0 = \frac{1}{B^2}I$ and $\wh\theta_{0,1/B^2} = \argmin_{\theta}\{\frac{1}{2B^2}\|\theta\|_2^2\} = 0$.

\subsection{Elliptical Potential Stuff}
\label{app::sec:elliptical_potential}

Here, we go through the elliptical potential stuff from \citet{abbasi2011improved} (also in \citet{lattimore2020bandit}) and say a bit about how it fits into the regret analysis of LinUCB/OFUL. We will assume that $\|\theta^*\|_2 \leq 1$ and $\max_{t}\|X_t\|_2 \leq 1$. As already mention in Section \ref{subsec:regret_analysis_standard}, we can bound the regret $r_t$ of LinUCB in round $t$ as
\begin{equation*}
r_t \leq 2\sqrt{\beta_{t-1}(\delta)}\min(1, \|X_t\|_{V_{t-1}^{-1}})\,.
\end{equation*}

We have established bounds on $\beta_t(\delta)$ already, so we only need to bound $\sum_{t=1}^{T}\min(1, \|X_t\|_{V_{t-1}^{-1}})$. The elliptical potential lemma provides a bound on $\sum_{t=1}^{T}\min(1, \|X_t\|_{V_{t-1}^{-1}}^2)$, which would allow us to bound $\sum_{t=1}^{T}r_t^2$. We can relate $\sum_{t=1}^{T}r_t$ to $\sum_{t=1}^{T}r_t^2$ in two ways. First, we can use the Cauchy-Schwarz inequality to obtain
\begin{equation*}
\sum_{t=1}^{T}r_t \leq \sqrt{T\sum_{t=1}^{T}r_t^2}\,.
\end{equation*}

This will lead to a regret bound of order $\mathcal{O}(p\sqrt{T}\log(T))$. If we know that there is a positive gap between the reward of the best and second best actions in every round, then we can do something else. Let $X_t^* = \argmax_{x \in \mathcal{X}_t}\iprod{\theta^*}{x}$ and define $\Delta = \min_{t \in [T]}\min_{x \in \mathcal{X}_t\setminus\{X_t^*\}}\{\iprod{\theta^*}{X_t^* - x}\}$. We assume that $\Delta > 0$. In every round, we have either $r_t = 0$ or $r_t \geq \Delta$, which means
\begin{equation*}
\sum_{t=1}^{T}r_t \leq \frac{1}{\Delta}\sum_{t=1}^{T}r_t^2\,.
\end{equation*}

This leads to regret bounds of order $\mathcal{O}(\frac{p^2\log^2(T)}{\Delta})$ (or maybe $\mathcal{O}(\frac{p^2\log(T)}{\Delta})$). The only thing left is the elliptical potential lemma itself.



\subsection{Regret analysis in the standard setting}
\label{subsec:regret_analysis_standard}
\textit{In this subsection we can assume that $\X$ is the initial set of actions and remains the same for each round. A more general assumption where our results would still apply is to assume the actions sets are time-dependent but fixed in advance by an oblivious adversary. Also we will assume $\dim(\X)=p$.}
\\

\noindent
Now that we have built our confidence sequence we are ready to bound the regret. Let's start by recalling the regret definition : 
\[\Reg(T) = \sum_{t=1}^T \langle X_t^*-X_t,\theta^*\rangle\]
The standard analysis follows from \cite{abbasi2011improved} and consists in two main steps.
\\

\noindent The first one focuses on bounding the instantaneous regret $r_t := \langle X_t^*-X_t,\theta^*\rangle.$ We have the following : 
    \begin{align*}
        r_t &= \langle X_t^*,\theta^*\rangle - \langle X_t,\theta^*\rangle\\
        &\leq \langle X_t,\theta_t\rangle - \langle X_t,\theta^*\rangle \qquad \qquad \text{(since $(X_t,\theta_t) = \argmax_{(x,\theta) \in \mathcal{X_t} \times C_{t-1}(\delta)} \langle x,\theta\rangle $)} \\
        &= \langle x_t,\theta_t - \hat \theta_t \rangle + \langle x_t,\hat \theta_t - \theta^*\rangle \\
        &\leq 2\beta_{t}(\delta)||X_t||_{\bar C_{t-1}^{-1}} \qquad \qquad \text{(applying Cauchy-Schwarz )}
    \end{align*}
   Here $\beta_t(\delta)\geq ||\wh \theta_{t-1} - \theta^*||_{V_{t-1}}$ is the width of the $C_t(\delta)$ centered around $\wh \theta_{t-1}:= V_{t-1}^{-1}\sum_{s=1}^{t-1}Y_sX_s=\theta^*+V_{t-1}^{-1}\sum_{s=1}^{t-1}\epsilon_tX_t$.
The last part of this step is to bound the norm of the actions. The technique is also refers to as the Elliptical potential lemma which we state below.
